HATS-74Ab, HATS-75b, HATS-76b and HATS-77b: Four Transiting Giant Planets around K and M Dwarfs

The relative rarity of giant planets around low mass stars compared with solar-type stars is a key prediction from core accretion planet formation theory. In this paper we report on the discovery of four gas giant planets that transit low mass late K and early M dwarfs. The planets HATS-74Ab (TOI 737b), HATS-75b (TOI 552b), HATS-76b (TOI 555b), and HATS-77b (TOI 730b), were all discovered from the HATSouth photometric survey and followed-up using TESS and other photometric facilities. We use the new ESPRESSO facility at the VLT to confirm and systems and measure their masses. We find that that planets have masses of 1.46 +- 0.14 MJ , 0.491 +- 0.039 MJ , 2.629 +- 0.089 MJ and 1.374 +0.100-0.074 MJ , respectively, and radii of 1.032 +- 0.021 RJ , 0.884 +- 0.013 RJ , 1.079 +- 0.031 RJ , and 1.165 +- 0.021 RJ, respectively. The planets all orbit close to their host stars with orbital periods ranging from 1.7319 d to 3.0876 d. With further work we aim to test core accretion theory by using these and further discoveries to quantify the occurrence rate of giant planets around low mass host stars.

==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxB below with a unique identifier for each planet (e.g. xxxxB for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxB. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxB}{HATS-40}
\newcommand{\hatcurbxxxxB}{HATS-40b}
\newcommand{\hatcurcxxxxB}{HATS-40c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxB}{40}

\newcommand{\hatcurCCtwomassshortxxxxB}{06421710-2946365}

%\newcommand{\hatcurCCraxxxxB}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxB}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxB}{\hatcurRVgamma{\hatcurplanetnumxxxxB}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxB}{\hatcurRVgamma{\hatcurplanetnumxxxxB}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxB}{\ensuremath{NULL\pm NULL}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxB}{i}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxB}{YY}
%\newcommand{\hatcurisoshortxxxxB}{Baraffe}
\newcommand{\hatcurisofullxxxxB}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxB}{Baraffe}
\newcommand{\hatcurisocitexxxxB}{yi:2001}
%\newcommand{\hatcurisocitexxxxB}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxB}{\arstar}
%\newcommand{\hatcurlumindxxxxB}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxB}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxB}{BB}
%\newcommand{\hatcurjhkfilsetxxxxB}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxBx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxB}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEzfehxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxB}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEzfehshortxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxB}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEloggxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxB}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvsinxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxB}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvmacxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxB}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvmicxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxB}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxB}}}

